A critical layer model for turbulent pipe flow

A model-based description of the scaling and radial location of turbulent fluctuations in turbulent pipe flow is presented and used to illuminate the scaling behaviour of the very large scale motions. The model is derived by treating the nonlinearity in the perturbation equation (involving the Reynolds stress) as an unknown forcing, yielding a linear relationship between the velocity field response and this nonlinearity. We do not assume small perturbations. We examine propagating modes, permitting comparison of our results to experimental data, and identify the steady component of the velocity field that varies only in the wall-normal direction as the turbulent mean profile. The "optimal" forcing shape, that gives the largest velocity response, is assumed to lead to modes that will be dominant and hence observed in turbulent pipe flow. An investigation of the most amplified velocity response at a given wavenumber-frequency combination reveals critical layer-like behaviour reminiscent of the neutrally stable solutions of the Orr-Sommerfeld equation in linearly unstable flow. Two distinct regions in the flow where the influence of viscosity becomes important can be identified, namely a wall layer that scales with $R^{+1/2}$ and a critical layer, where the propagation velocity is equal to the local mean velocity, that scales with $R^{+2/3}$ in pipe flow. This framework appears to be consistent with several scaling results in wall turbulence and reveals a mechanism by which the effects of viscosity can extend well beyond the immediate vicinity of the wall.

==> ModeAmp.tex <==
\section{Mode amplification}\label{sect:subamp}

The range of modes that are observed in practice will depend on the product of the response, i.e. $\sigma$, and the initial forcing amplitude, $|f|$.  With this caveat in mind, there is excellent agreement between the predictions of our model shown in the earlier figures and the shape of the most amplified propagating POD modes in the work of Duggleby \etal. We consider now the variation of the amplitude of the velocity response for unit forcing, with a focus on the wavenumber pairs of known interest to high Reynolds number wall turbulence.

\begin{figure}
\begin{center}
\includegraphics[width = 12cm]{sigma1_lxp1000lzp100_Res.eps}
\caption{Variation of the first singular value, $\sigma_1$, with Reynolds number for the $(\lambda_x^+,\lambda_z^+)=(1000,100)$ mode.}
\end{center}
\label{fig:ampwall}
\end{figure}
% plot_sigma_var.m

\begin{figure}
\begin{center}
\includegraphics[width = 12cm]{sigma1_k1n10_Res.eps}
\caption{Variation of the first singular value, $\sigma_1$, with Reynolds number for the $(k,n)=(1,10)$ mode.}
\end{center}
\label{fig:ampVLSM}
\end{figure}
% plot_sigma_var.m

Figure~\ref{fig:VLSM_growth}

Figures~\ref{fig:ampwall} and~\ref{fig:ampVLSM} show the variation of the first singular value with streamwise wavespeed as a function of Reynolds numbers for the near-wall and VLSM wavenumber pairs identified above.  Interestingly, these modes show opposite trends with increasing Reynolds number.  For the near-wall mode, the singular values decrease as a function of Reynolds number such that $\sigma_1 < 1$ for all wavespeeds when $Re \gtrsim 4.1 \times 10^5$.  At all Reynolds numbers the response drops off rapidly as the streamwise wavespeed approaches the centreline velocity, as would be expected.

For the VLSM mode, increasing the Reynolds number increases the peak response amplitude such that $\sigma_{VLSM, max} \sim R^+ ******$, while the response is approximately Reynolds number independent (and small) for $U/U_{CL} \lesssim 0.4$ and $\gtrsim 1$.

\bjm{Maximum growth still occurs for low $k$ - CHECK.  Take a look at surface plots with different $(k,n,\omega)$ at a couple of Reynolds numbers.}

We note that the results from the initial value problem in turbulent channel~\cite{delAlamo06} and boundary layer flow~\cite{Cossu09}, as well as in the laminar channel~\cite{Jovanovic05} indicate that the response modes correspond to the largest energy amplification always correspond to streamwise-constant, $k=0$, modes. The approach described here is still an input-output analysis, but differs by considering only (orthogonal) harmonic forcing and response pairs with the forcing derived from the non-linear terms in the Navier-Stokes equations (such that the wavenumbers where significant forcing occurs can be closely linked with the spectral ranges containing significant kinetic energy).  In addition, the influence of the wavespeed permits us to make analogy to critical layer theory in laminar flow.  We stress again that this analysis explicitly cannot treat modes with $k$ or $n=0$, \bjm{but note that the trends exhibited in figures~\ref{fig:sigmasurflxp1} and \ref{fig:sigmasurfV1} indicate an increasing level of response for decreasing streamwise wavenumber.  NEED TO CHECK THIS - IT WAS NOT ALWAYS THE CASE WHEN N WAS CHANGED}.

Figure~\ref{fig:sigmasurflxp2}...

\begin{figure}
\begin{center}
\includegraphics[width = 14cm]{sigma1_lxp1000.eps}
\label{fig:sigmasurflxp1}
\caption{Variation of the first singular value, $\sigma_1$, with azimuthal wavenumber for the $(k,\omega)=(2\pi R^+/1000,10 k u_\tau)$ mode at $Re=75 \times 10^3$. Note that this curve is not truly continuous since the pipe geometry imposes the constraint of integer $n$: symbols correspond to the integer azimuthal wavenumbers for which $\sigma_1$ is calculated.}
\end{center}
\end{figure}
% plot_sigma_var_ws.m

\begin{figure}
\begin{center}
\includegraphics[width = 14cm]{sigma1_lxp.eps}
\label{fig:sigmasurflxp2}
\caption{Variation of the first singular value, $\sigma_1$, with azimuthal wavenumber for $(\omega)=(10 k u_\tau)$ mode at $Re=75 \times 10^3$. From the lowest to the highest curve: $\lambda_x^+ = 10,100,1000,10000,23050$.}
\end{center}
\end{figure}
% plot_sigma_var_ws.m

\begin{figure}
\begin{center}
\includegraphics[width = 14cm]{sigma1_k1.eps}
\label{fig:sigmasurfV1}
\caption{Variation of the first singular value, $\sigma_1$, with azimuthal wavenumber for the $(k,\omega)=(1,0.67 U_{CL})$ mode at $Re=75 \times 10^3$.  Note that this curve is not truly continuous since the pipe geometry imposes the constraint of integer $n$: symbols correspond to the integer azimuthal wavenumbers for which $\sigma_1$ is calculated.}
\end{center}
\end{figure}
% plot_sigma_var_ns.m






